Functional SDE approximation inspired by a deep operator network architecture

A novel approach to approximate solutions of Stochastic Differential Equations (SDEs) by Deep Neural Networks is derived and analysed. The architecture is inspired by the notion of Deep Operator Networks (DeepONets), which is based on operator learning in function spaces in terms of a reduced basis also represented in the network. In our setting, we make use of a polynomial chaos expansion (PCE) of stochastic processes and call the corresponding architecture SDEONet. The PCE has been used extensively in the area of uncertainty quantification (UQ) with parametric partial differential equations. This however is not the case with SDE, where classical sampling methods dominate and functional approaches are seen rarely. A main challenge with truncated PCEs occurs due to the drastic growth of the number of components with respect to the maximum polynomial degree and the number of basis elements. The proposed SDEONet architecture aims to alleviate the issue of exponential complexity by learning an optimal sparse truncation of the Wiener chaos expansion. A complete convergence and complexity analysis is presented, making use of recent Neural Network approximation results. Numerical experiments illustrate the promising performance of the suggested approach in 1D and higher dimensions.

==> sections/remarks.tex <==
\setcounter{section}{-1}
\section{Remarks}

Referee \#1 (Remarks to the Author):

The authors aim to solve stochastic differential equations driven by Brownian motion by using operator neural networks. These networks learn the solution map that takes the Brownian motion path to the solution of the stochastic differential equation (SDEs).

The key idea is based on the polynomial chaos expansion of the SDE solution, see equations (2.6), (2.9) and (3.5). In this expansion, the authors compute the Brownian integrals (lines 343-344), but approximate the Wiener chaos polynomials and the coefficients by neural networks.

In Section 4 the authors then provide an approximation error analysis and obtain bounds on the $L^2$-error between the SDE solution and the neural network approximation. Lemma 4.3 decomposes this error into three terms: truncation, approximation and reconstruction errors. The first term is analysed based on truncation error bounds for Wiener chaos expansions from the literature (Theorem 2.5). The second term is bounded in Lemma 4.9. The proof proceeds by bounding the coefficients in the Wiener chaos expansion (Lemma 4.8) using the Malliavin derivatives of the underlying process. The last error term is then bounded in Lemma 4.12 using ReLU DNN approximation bounds from the literature. At the end the article also contains numerical simulation results.

In general, the article contains an interesting new idea. However, \textcolor{red}{I have a major concern about the relevance of the method. The considered SDEs can be simulated very efficiently by an Euler-Maruyama scheme. Under the hypotheses formulated in Assumption 1 the Euler scheme converges strongly with dimension-free convergence rates and explicit constants. The Euler scheme can be implemented very easily and works very well also in higher dimensions. It thus provides a natural and simple way of simulating these processes. On the other hand, the proposed method requires training large neural networks and leads to trajectories that do not capture important roughness properties of the sample path of the stochastic processes of interest (see Figure 5). Thus, I don't see a convincing reason why the proposed method could be useful in comparison to just employing a standard Euler scheme.}

I think that the results are interesting and should be published. However, given that there is no benefit from using the proposed networks as compared to simply employing an Euler scheme, I don't think that the results are at the level required for a top journal such as SINUM.

Finally, an additional comment on the main error bound: in \textcolor{red}{the main error bound in Theorem 4.1 the right hand side of the bound still depends on the L2-norm of the neural networks approximating the basis (see line 374). In particular, we can not use the bound to actually understand the network size needed to achieve a given approximation accuracy epsilon $\varepsilon$ this makes the analysis somewhat incomplete.}

Some minor comments:
\begin{itemize}
    \item In the introduction the authors write: \textcolor{red}{"The convergence rate depends directly on the regularity of the SDE, and hence is quite limited by the typical lack thereof." What do the authors mean by this? Here they also assume regularity for the coefficients of the SDE}.
    \item It is unclear how Example 3.9 is to be understood. A stochastic integral can not be defined pathwise in general. That is, the map $\omega \mapsto \int_0^t H_s dW_s(\omega)$ is not well-defined for general bounded H. Possibly for this choice of H it is? I think this would need to be clarified.
\end{itemize}

% TODOS

\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\writing}{\textcolor{RoyalBlue}{{{\large\hspace{1pt}\ding{45}}}}}
\newcommand{\done}{\textcolor{ForestGreen}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}}}%

\textbf{\textcolor{red}{TODOs:}}
\begin{todolist}
    \item[\done] Motivate the use of this architecture over the Euler-Maruyama scheme,
    \begin{itemize}
        \item with our assumptions, the Euler scheme work very well in high dimensions,
        \item our method needs the training of large neural networks,
        \item do not capture important roughness properties of the sample path of the stochastic processes
        \item \charles{We can think of the case where the drift and/or the diffusion is/are unknown}
        \item \charles{We can also think about SPDEs e.g. stochastic eat equation, Burger. We could fix the spatial variable. Make an outlook on the extension using Wuan Luo's work.}
    \end{itemize}
    \item[\done] RHS of Theorem 4.1 still depends on the $L^2$-norm of the NNs approximating the basis,
    \begin{itemize}
        \item \charles{We can use the approximation of the $\widetilde\Psi_j$, and the orthonormality of the $\Psi_\alpha$}
        \item \charles{Since $\sum_{j=1}^p \E[\widetilde\Psi_j^2] = \sum_{j=1}^p \E[|\widetilde\Psi_j - \Psi_{k_j^*} + \Psi_{k_j^*}|^2] \leq 2(\varepsilon + p)$}
        \item \charles{Therefore, $\sqrt{\sum_{j=1}^p \E[\widetilde\Psi_j^2]} \leq \sqrt{2(\varepsilon+p)}$}
    \end{itemize}
    \item[\done] Example 3.9 is not clear: a stochastic integral cannot be defined pathwise in general
    \begin{itemize}[label=$\rightarrow$]
        \item \charles{Indeed, for almost all $\omega$, the function $s \mapsto B_s(\omega)$ is of unbounded variation, so we cannot consider the integral as an ordinary Riemann-Stieljes integral} \url{https://math.stackexchange.com/questions/3517080/what-mean-that-it%C3%B4-integral-is-not-pathwise-defined}
        \item \charles{Therefore, I suggest to remove any dependence on $\omega$.}
    \end{itemize}
\end{todolist}
